Sociotechnical Harms of Algorithmic Systems: Scoping a Taxonomy for Harm Reduction

Understanding the landscape of potential harms from algorithmic systems enables practitioners to better anticipate consequences of the systems they build. It also supports the prospect of incorporating controls to help minimize harms that emerge from the interplay of technologies and social and cultural dynamics. A growing body of scholarship has identified a wide range of harms across different algorithmic technologies. However, computing research and practitioners lack a high level and synthesized overview of harms from algorithmic systems. Based on a scoping review of computing research $(n=172)$, we present an applied taxonomy of sociotechnical harms to support a more systematic surfacing of potential harms in algorithmic systems. The final taxonomy builds on and refers to existing taxonomies, classifications, and terminologies. Five major themes related to sociotechnical harms - representational, allocative, quality-of-service, interpersonal harms, and social system/societal harms - and sub-themes are presented along with a description of these categories. We conclude with a discussion of challenges and opportunities for future research.

==> tablesAndFigures/allocativedatasources.tex <==
\begin{center}
\begin{longtable}{p{5cm}p{8cm}}
\caption{Allocative harms described in data sources.}
\label{allocativesources}\\
\toprule
Sub-type & References  \\ \midrule
Allocative harms (generally) & \cite{Angwin_Parris_2016, Bailey_Burkell_Dunn_Gosse_Steeves_2021, Balayn_Lofi_Houben_2021, Bandy2021, barocas-hardt-narayanan, binns2021, Blodgett_Barocas_Daume_Wallach_2020, Castillo_2019, cave2019bridging, corry2021problem, Davis_Williams_Yang_2021, Devinney_2022, Dev_Monajatipoor_Ovalle_Subramonian_Phillips_Chang_2021, Dobbe_Dean_Gilbert_Kohli_2018, Ekstrand_Das_Burke_Diaz_2022, Field_Blodgett_Waseem_Tsvetkov_2021, galaz2021artificial, galaz2021machine, Hoffmann_2021, Holstein_2019, Jacobs_2021, Jane_2018, Kaminski_Malgieri_2020, Kapania_Siy_Clapper_Sp_Sambasivan_2022, Knox_2019, Lloyd_2018, Luccioni_Corry_Sridharan_Ananny_Schultz_Crawford_2022, Mannes_2020, Markl_2022, Mashhadi_Zolyomi_Quedado_2022, Onuhoha, Ramesh_Kameswaran_Wang_Sambasivan_2022, Richardson_Gilbert_2021, Savoldi_Gaido_Bentivogli_Negri_Turchi_2021, Singh_Joachims_2018, Sun_Asudeh_Jagadish_Howe_Stoyanovich_2019, Suresh_Guttag_2021, Tufekci_Rit_Adam_Kramer_Guillory_Hancock, vanEs_2021, Weidinger2022, Weinberg_2022, Wu_Mitra_Ma_Diaz_Liu_2022, Yee_Tantipongpipat_Mishra_2021, Zajko_2022, rekabsaz2021, Metcalf_Moss_Watkins_Singh_Elish_2021} \\ \midrule
Opportunity loss & {Education discrimination}: ~\cite{Altman_Wood_Vayena_2018, Ehsan_Singh_Metcalf_Riedl_2022, Karumbaiah_Brooks_2021, Mashhadi_Zolyomi_Quedado_2022, microsoft_2020, Monroe-White_2021}; {Inequitable access to information/resources needed to participate in society}: \cite{cave2019bridging, Costanza-Chock_Raji_Buolamwini_2022, Kapania_Siy_Clapper_Sp_Sambasivan_2022, Markl_2022, Obermeyer_2019, Redden_Brand_2017}; {Housing discrimination}: ~\cite{Angwin_Parris_2016, Mashhadi_Zolyomi_Quedado_2022, Redden_Brand_2017, vanEs_2021, microsoft_2020} \\ \midrule

Economic loss & {Credit discrimination} \cite{Bandy2021, Jane_2018, Kapania_Siy_Clapper_Sp_Sambasivan_2022, Sambasivan_Arnesen_Hutchinson_Doshi_Prabhakaran_2021, Mannes_2020, Markl_2022, microsoft_2020, Monroe-White_2021, Redden_Brand_2017, Sambasivan_Arnesen_Hutchinson_Doshi_Prabhakaran_2021}; {Demonetization} \cite{Caplan_Gillespie_2020}; {Employment discrimination} \cite{Altman_Wood_Vayena_2018, DeVos_Dhabalia_Shen_Holstein_Eslami_2022, Jacobs_2021, koenecke2020racial, Krafft_2021, Lloyd_2018, microsoft_2020, Sambasivan_Arnesen_Hutchinson_Doshi_Prabhakaran_2021, Yee_Tantipongpipat_Mishra_2021}; {Financial injuries} \cite{Altman_Wood_Vayena_2018, Avila_2018, Dobbe_Krendl_Gilbert_Mintz_2021, Kapania_Siy_Clapper_Sp_Sambasivan_2022, Sambasivan_Arnesen_Hutchinson_Doshi_Prabhakaran_2021, Ramesh_Kameswaran_Wang_Sambasivan_2022, CSETTaxonomy, Metcalf_Moss_Watkins_Singh_Elish_2021}; {Insurance discrimination} \cite{Costanza-Chock_Raji_Buolamwini_2022, microsoft_2020}; {Loss of job opportunities} \cite{Altman_Wood_Vayena_2018, Krafft_2021, Mannes_2020, Wu_Mitra_Ma_Diaz_Liu_2022, Yee_Tantipongpipat_Mishra_2021}; {Price discrimination} \cite{Bandy2021, Chen_Mislove_Wilson_2016, microsoft_2020, Obermeyer_2019, Pandey_Caliskan_2021}\\ \hline
\end{longtable}
\end{center}


==> tablesAndFigures/excludedsources.tex <==
%\vspace{10mm}
\newpage
%\begin{center}
\begin{longtable}{@{} p{.75cm}p{4.5cm}p{7.5cm}p{3cm}}
\caption{Excluded sources.}
\label{Excluded sources}
\\
\toprule
Year & Author(s) & Title & Reason for Exclusion \\ \midrule
1993 & Kernohan, A. & Accumulative Harms and the Interpretation of the Harm Principle & Does not describe algorithmic systems \\ \hline
2008 & Klaus-Dieter, S., \& Thalheim, B. & Storyboarding Concepts for Edutainment WIS & Not focused on algorithmic system harms \\ \hline
2016 & Fiesler, C., Wisniewski, P., Pater, J., \& Andalibi, N. & Exploring Ethics and Obligations for Studying Digital Communities & Call for papers \\ \hline
2018 & Garvey, C. & AI Risk Mitigation Through Democratic Governance: Introducing the  7-Dimensional AI Risk Horizon & Full-text not available \\ \hline
2018 & Walker, W. & "Data Justice" By Design: Building Engagement Through Civic Technologies & Full-text not available \\ \hline
2018 & Passi, S., \& Jackson, S.J. & Trust in Data Science: Collaboration, Translation, and Accountability in Corporate Data Science Projects & Not focused on algorithmic system harms \\ \hline
2018 & Veale, M., Van Kleek, M., \& Binns, R. & Fairness and Accountability Design Needs for Algorithmic Support in High-Stakes Public Sector Decision-Making & Not focused on algorithmic system harms \\ \hline
2019 & Rempel, E., Barnett, J., \& Durrant, H. & Contrasting Views of Public Engagement on Local Government Data Use in the UK & Not focused on algorithmic system harms \\ \hline
2019 & Ekstrand, M.D., Burke, R., \& Diaz, F. & Fairness and Discrimination in Recommendation and Retrieval in RecSys ‘19 & Full-text not available \\ \hline
2019 & Ekstrand, M.D., Burke, R., \& Diaz, F. & Fairness and Discrimination in Recommendation and Retrieval in SIGIR ‘19 & Full-text not available \\ \hline
2020 & Cath, C., Latonero, M., Marda, V., \& Pakzad, R. & Leap of FATE: Human Rights as a Complementary Framework for AI Policy and Practice & Conference tutorial \\ \hline
2020 & Dias, V., Lokanathan, S., \& Wijeratne, Y. & A Brief Primer on Bias in Machine Learning and Algorithmic Decisions [White Paper] & Full-text source available is incomplete \\ \hline
2020 & Theodorou, A., \& Dignum, V. & Towards Ethical and Socio-legal Governance in AI. & Full-text source unavailable \\ \hline
2020 & Baker, D., Hanna, A., \& Denton, E. & Algorithmically Encoded Identities: Reframing Human Classification & Full-text source unavailable \\ \hline 
2020 & Jacobs, A.Z., Blodgett, S.L., Barocas, S., Daumé, H., \& Wallach, H. & The Meaning and Measurement of Bias: Lessons from Natural Language Processing & Conference tutorial \\ \hline
2020 & Zhuang, W., Wen, Y., Zhang, X., Gan, X., Yin, D., Zhou, D., Zhang, S., \& Yi, S. & Performance Optimization of Federated Person Re-identification via Benchmark Analysis & Not focused on algorithmic system harms \\ \hline
2021 & Metaxa, D., Park, J., Robertson, R., Karahalios, K., Wilson, C., Hancock, J., \& Sandvig, C. & Auditing Algorithms: Understanding Algorithmic Systems from the Outside In & Focused on machine behaviors, rather than harms \\ \hline
2021 & Watkins, E., Moss, E., Metcalf, J., Singh, R., \& Elish, M. & Governing Algorithmic Systems with Impact Assessments: Six Observations & Focused on Impact Assessments \\ \hline
2021 & Zhou, F., Yu, L., Xu, X., \& Trajcevski, G. & Decoupling Representation and Regressor for Long-Tailed Information Cascade Prediction & Focused on harm to models, rather than harms from models \\ \hline
2021 & Hanna, J.P., Niekum, S., \& Stone, P. & Importance Sampling in Reinforcement Learning with an Estimated Behavior Policy & Not focused on algorithmic system harms \\ \hline
2021 & Whittaker, M. & The Steep Cost of Capture & Not focused on harms from algorithmic systems \\ \hline
2021 & Gaikwad, S.N., Iyer, S., Lunga, D., \& Bondi, E. & Data-driven Humanitarian Mapping: Harnessing Human-Machine Intelligence for High-Stake Public Policy and Resilience Planning & Full-text not available \\ \hline
2021 & Benitez, Y.S. & Algorithmic Ecologies of Justice: Using Computational Social Science Methods to Co-design Tools of Resistance, Resilience and Care with Communities & Full-text not available \\ \hline
2022 & Birhane, A., Kalluri, P., Card, D., Agnew, W., Dotan, R., \& Bao, M. & The Values Encoded in Machine Learning Research & Not focused on algorithmic system harms \\ \hline
2022 & Abdellatif, A., Mhaisen, N., Mohamed, A., Erbad, A., Guizani, M., Dawy, Z., \& Nasreddine, W. & Communication-efficient Hierarchical Federated Learning for IoT Heterogeneous Systems with Imbalanced Data & Not focused on algorithmic system harms \\ \hline
2022 & Shah, C., Suel, T., Diaz, F., Mitra, B., Poblete, B., Suleman, H., \& Verberne, S. &
Report on the 44th International ACM SIGIR Conference on Research and Development in Information Retrieval & Not focused on algorithmic system harms \\ \hline
2022 & Berridge, C., Zhou, Y., Lazar, A., Porwal, A., Mattek, N., Gothard, S., \& Kaye, J. &
Control Matters in Elder Care Technology: Evidence and Direction for Designing IT & Not focused on algorithmic system harms \\ \hline
2022 & Olewicki, D., Nayrolles, M., \& Adams, B. & Towards Language-independent Brown Build Detection & Focused on harm to models, rather than harms from models \\ \hline
2022 & Hamed, I., Denisov, P., Li, C., Elmahdy, M., Abdennadher, S., \& Vu, N. & Investigations on Speech Recognition Systems for Low-resource Dialectal Arabic–English Code-switching Speech & Not focused on algorithmic system harms \\ \hline
2022 & Lum, K., Zhang, Y., \& Bower, A. & De-biasing “Bias” Measurement & Not focused on algorithmic system harms \\ \hline
2022 & Zhang, L., Lu, X., Chen, Z., Liu, T., Chen, Q., \& Li, Z. & Adaptive Deep Learning for Network Intrusion Detection by Risk Analysis & Not focused on algorithmic system harms \\ \hline
2022 & Young, M., Katell, M., \& Krafft, P.M. & Confronting Power and Corporate Capture at the FAccT Conference & Not focused on algorithmic system harms \\ \hline
2022 & Howard, N., Madkins, T., \& White, S.V. & Disrupting Anti-Blackness While Making Room for Black Girls and Women in CS and Tech & Full-text not available \\ \hline
2022 & Blodgett, S.L., Liao, Q.V., Olteanu, A., Mihalcea, R., Muller, M., Scheuerman, M.K., Tan, C., \& Yang, Q. & Responsible Language Technologies: Foreseeing and Mitigating Harms & Full-text not available \\ \hline
2022 & Li, Z., Nie, J., Song, Y., Du, P., \& Li, D. & Learning to Classify Relations Between Entities from Noisy Data - A Meta-Instance Reweighting Approach & Not focused on algorithmic system harms
\end{longtable}
%\end{center}


==> tablesAndFigures/interpersonaldatasources.tex <==
\newpage
\begin{longtable}{{p{5cm}p{8.5cm}}}
\caption{Interpersonal harms described in data sources.}
\label{interpersonalsources}\\
\toprule
Sub-type & References  \\ \midrule
Loss of agency / Social control & Agency loss / Social control (generally): ~\cite{Dean_Gilbert_Lambert_Zick_2021, McGlynn_Rackley_2017,  Malik_Viljanen_Lepinkainen_Alvesalo-Kuusi_Others, Mann_Matzner_2019, Keyes_2018, Wang_2020,Agrafiotis_Nurse_Goldsmith_Creese_Upton_2018, Smuha_2021a, Karizat_2021, Andalibi_Garcia_2021, Skirpan_Fiesler_2018, Lustig_Konrad_Brubaker_2022, Bandy2021, Tufekci_Rit_Adam_Kramer_Guillory_Hancock, Weidinger2022, Thiago_Marcelo_Gomes_2021, Mohamed_Png_Isaac_2020, microsoft_2020, Bailey_Burkell_Dunn_Gosse_Steeves_2021, Birhane_Prabhu_Kahembwe_2021, Wang_Zhao_Van_Kleek_Shadbolt_2022, Moss_2021}; Algorithmically-informed identity change: ~\cite{Karizat_2021}\\ \midrule

Technology-facilitated violence & Technology-facilitated violence (generally): ~\cite{Brown_Sanci_Hegarty_2021, Freed_Palmer_Minchala_Levy_Ristenpart_Dell_2018, Henry_Flynn_Powell_2020, Bailey_Henry_Flynn_2021, Dev_Monajatipoor_Ovalle_Subramonian_Phillips_Chang_2021, Keyes_2018, Holstein_2019, Alkhatib2021, Scheuerman_Branham_Hamidi_2018, Wang_Zhao_Van_Kleek_Shadbolt_2022, Moss_2021};
Coercive control, or intimate partner violence: ~\cite{Dragiewicz_2018, Henry_Flynn_Powell_2020}; Inciting or enabling offline violence: ~\cite{Moss_2021, Tufekci_Rit_Adam_Kramer_Guillory_Hancock}; Online abuse (e.g., bullying, deadnaming, doxxing, trolling, hateful or toxic language): ~\cite{Maity_Chakraborty_Goyal_Mukherjee_2018, Vitak_Chadha_Steiner_Ashktorab_2017, Sheth_Shalin_Kursuncu_2021, Guberman_Schmitz_Hemphill_2016, Slonje_Smith_Frisen_2013, Ayodeji_Olamijuwon_Kokomma_Onyemelukwe_Gboyega_2021, Douglas_2016, Freed_Palmer_Minchala_Levy_Ristenpart_Dell_2018, Scheuerman_Jiang_Fiesler_Brubaker_2021, Ramesh_Kameswaran_Wang_Sambasivan_2022, Lloyd_2018, Feder_Cooper_Moss_Laufer_Nissenbaum_2022, brundage2018malicious, Scheuerman_Branham_Hamidi_2018, Sambasivan_Arnesen_Hutchinson_Doshi_Prabhakaran_2021, modei_Olah_Steinhardt_Christiano_Schulman_Mane_2016, Wang_Zhao_Van_Kleek_Shadbolt_2022}; Online sexual harassment (e.g., image-based abuse, cyberstalking, sexual harassment, sextortion): ~\cite{Ayodeji_Olamijuwon_Kokomma_Onyemelukwe_Gboyega_2021, Douglas_2016, Freed_Palmer_Minchala_Levy_Ristenpart_Dell_2018, Dragiewicz_2018, Henry_Flynn_Powell_2020, Ramesh_Kameswaran_Wang_Sambasivan_2022, Bandy2021, Altman_Wood_Vayena_2018, McGlynn_Rackley_2017, Sambasivan_Arnesen_Hutchinson_Doshi_Prabhakaran_2021, Henry_Flynn_Powell_2020, Bailey_Burkell_Dunn_Gosse_Steeves_2021} \\ \midrule

Diminished health and well-being & 
{Behavioral manipulation:} ~\cite{Karizat_2021, microsoft_2020}; Emotional harms (e.g., dignity loss, invalidation, misgendering): ~\cite{Bengio_Beygelzimer_Crawford_Fromer_Gabriel_Levendowski_Raji_Ranzato_2022, Wardle_and_Derakhshan_2017, Cambre_Kulkarni_2019, Karizat_2021, McGlynn_Rackley_2017, Agrafiotis_2016, Redden_Brand_2017, Scheuerman_Branham_Hamidi_2018, Vitak_Chadha_Steiner_Ashktorab_2017, Brown_Sanci_Hegarty_2021, Jane_2018, Mannes_2020, Dev_Monajatipoor_Ovalle_Subramonian_Phillips_Chang_2021, Keyes_2018, Thiago_Marcelo_Gomes_2021, Welbl_2021, Andalibi_Garcia_2021, Weidinger2022, Bandy2021, Feder_Cooper_Moss_Laufer_Nissenbaum_2022, brundage2018malicious, microsoft_2020, CSETTaxonomy, Wang_2020}; Physical harms: ~\cite{Bengio_Beygelzimer_Crawford_Fromer_Gabriel_Levendowski_Raji_Ranzato_2022, Wardle_and_Derakhshan_2017, Cambre_Kulkarni_2019, Karizat_2021, McGlynn_Rackley_2017, Agrafiotis_2016, Redden_Brand_2017, Mannes_2020, Scheuerman_Branham_Hamidi_2018, Vitak_Chadha_Steiner_Ashktorab_2017, Brown_Sanci_Hegarty_2021, Douglas_2016, Bennett_Gleason_Scheuerman_Bigham_Guo_To_2021, Scheuerman_Jiang_Fiesler_Brubaker_2021, Pendse2022, Ramesh_Kameswaran_Wang_Sambasivan_2022, DeVos_Dhabalia_Shen_Holstein_Eslami_2022, microsoft_2020, CSETTaxonomy, Wang_Ramaswamy_Russakovsky_2022}; Reputational harms: ~\cite{Redden_Brand_2017, Bennett_Gleason_Scheuerman_Bigham_Guo_To_2021, Png_2022, CSETTaxonomy, Metcalf_Moss_Watkins_Singh_Elish_2021, Moss_2021, Agrafiotis_2016, Bailey_Burkell_Dunn_Gosse_Steeves_2021, Sanchez2021, Hutchinson2020socialbiases} \\ \midrule
Privacy violations & {Privacy violations (generally):} ~\cite{Bengio_Beygelzimer_Crawford_Fromer_Gabriel_Levendowski_Raji_Ranzato_2022, McGlynn_Rackley_2017, Redden_Brand_2017, Mannes_2020, Welbl_2021, Ehsan_Singh_Metcalf_Riedl_2022, Chancellor_2019, binns2021, Formosa_Wilson_Richards_2021, Chi_Lurie_Mulligan, Ekstrand_Das_Burke_Diaz_2022, Png_2022, Kaminski_Malgieri_2020, Weidinger2022, Slupska_Dawson_Duckworth_Ma_Neff_2021, Ramesh_Kameswaran_Wang_Sambasivan_2022, corry2021problem, Tufekci_Rit_Adam_Kramer_Guillory_Hancock, Birhane_2021, Dobbe_Krendl_Gilbert_Mintz_2021, Feder_Cooper_Moss_Laufer_Nissenbaum_2022, microsoft_2020, Moss_2021, Metcalf_Moss_Watkins_Singh_Elish_2021, Raji_Gebru_Mitchell_Buolamwini_Lee_Denton_2020, Bailey_Burkell_Dunn_Gosse_Steeves_2021, Wang_Zhao_Van_Kleek_Shadbolt_2022}; Algorithmic profiling: ~\cite{Mohamed_Png_Isaac_2020, Sambasivan_Arnesen_Hutchinson_Doshi_Prabhakaran_2021, Redden_Brand_2017, Mann_Matzner_2019, Monroe-White_2021}; Feelings of surveillance, or loss of desired anonymity: ~\cite{Rincon_Keyes_Cath_2021, Mann_Matzner_2019, Ehsan_Singh_Metcalf_Riedl_2022, Monroe-White_2021, Costanza-Chock_Raji_Buolamwini_2022, Krafft_2021, Markl_2022, Skirpan_Fiesler_2018, Katell_Young_Dailey_Herman_Guetler_Tam_Bintz_Raz_Krafft_2020, Slupska_Dawson_Duckworth_Ma_Neff_2021, van_der_Sloot_van_Schendel_2021}; Loss of right to be forgotten: ~\cite{Altman_Wood_Vayena_2018, Wang_Zhao_Van_Kleek_Shadbolt_2022}; Non-consensual data collection: ~\cite{Kapania_Siy_Clapper_Sp_Sambasivan_2022}; Privacy attacks (e.g., identity theft, doxxing): ~\cite{Redden_Brand_2017, Douglas_2016, Bandy2021} \\ \hline
\end{longtable}
%\end{center}


==> tablesAndFigures/qualitydatasources.tex <==
\begin{center}
\begin{longtable}{{p{5cm}p{8cm}}}
\caption{Quality-of-service harms described in data sources.}
\label{qosdatasources}\\
\toprule
Sub-type & References  \\ \midrule
Quality-of-service harms (generally) & 
\cite{binns2021,Buolamwini_Friedler_Wilson,DeVries_2019,Ekstrand_Das_Burke_Diaz_2022, joyce2021toward,Kaminski_Malgieri_2020, koenecke2020racial, Markl_2022, mengesha2021don, Obermeyer_2019, Raz_2021, Suresh_Guttag_2021, Rincon_Keyes_Cath_2021, Sambasivan_Arnesen_Hutchinson_Doshi_Prabhakaran_2021, Weidinger2022} \\ \midrule

Alienation & \cite{Bennett_Gleason_Scheuerman_Bigham_Guo_To_2021, Bivens_Haimson_2016, Blodgett_Barocas_Daume_Wallach_2020, Keyes_2018, Mannes_2020, mengesha2021don, Rincon_Keyes_Cath_2021, Weidinger2022} \\ \midrule

Increased labor & 
\cite{Bennett_Gleason_Scheuerman_Bigham_Guo_To_2021, Blodgett_Barocas_Daume_Wallach_2020, DeVos_Dhabalia_Shen_Holstein_Eslami_2022, koenecke2020racial, mengesha2021don} \\ \midrule
Service loss & {Algorithmic invisibility:} ~\cite{DeVries_2019, Duffy_Meisner_2022, Sambasivan_Arnesen_Hutchinson_Doshi_Prabhakaran_2021, Tatman_2017}; Degraded performance: ~\cite{aksenova-etal-2021-might,DeVries_2019,vanEs_2021,galaz2021machine, Hoffmann_2021, koenecke2020racial, Liao_2015, mengesha2021don, Obermeyer_2019, Tatman_2017} \\ \hline
\end{longtable}
\end{center}


==> tablesAndFigures/representationaldatasources.tex <==
%\newpage
\begin{center}
\begin{longtable}{p{5cm}p{8cm}}
\caption{Representational harms described in data sources.}
\label{representationaldatasources}\\
\toprule
Sub-type & References \\ \midrule
%\endfirsthead
%\toprule
%Harm Theme & Instances & References \\ \midrule
%\endhead 
%\endfoot
%\bottomrule 
%\endlastfoot
Representational harms (generally) &  \cite{Andalibi_Garcia_2021, Bailey_Burkell_Dunn_Gosse_Steeves_2021, Balayn_Lofi_Houben_2021, Bandy2021, Barabas_Doyle, barocas-hardt-narayanan, Bengio_Beygelzimer_Crawford_Fromer_Gabriel_Levendowski_Raji_Ranzato_2022, Birhane_Prabhu_Kahembwe_2021, Blodgett_Barocas_Daume_Wallach_2020, Castillo_2019, Chi_Lurie_Mulligan,corry2021problem, Davis_Williams_Yang_2021, DeVos_Dhabalia_Shen_Holstein_Eslami_2022, Dobbe_Dean_Gilbert_Kohli_2018, Ekstrand_Das_Burke_Diaz_2022, galaz2021artificial, galaz2021machine, Hendricks_Burns_Saenko_Darrell_Rohrbach_2018, Holstein_2019, Hutchinson_Prabhakaran_Denton_2020, Jane_2018, Karizat_2021, Katzman_Barocas_Blodgett_Laird_Scheuerman_Wallach_2021, Kay_Matuszek_Munson_2015, Knox_2019, Lloyd_2018, Luccioni_Corry_Sridharan_Ananny_Schultz_Crawford_2022, Mannes_2020, Markl_2022, Mashhadi_Zolyomi_Quedado_2022, Monroe-White_2021, Paullada_Raji_Bender_Denton_Hanna_2021,  Pruksachatkun_Krishna_Dhamala_Gupta_Chang_2021,Richardson_Gilbert_2021, Rincon_Keyes_Cath_2021, Savoldi_Gaido_Bentivogli_Negri_Turchi_2021, Sun_Asudeh_Jagadish_Howe_Stoyanovich_2019, Sweeney_2013, vanEs_2021, Wang_Barocas_Laird_Wallach_2022, Weidinger2022, Weinberg_2022, Wu_Mitra_Ma_Diaz_Liu_2022, Yee_Tantipongpipat_Mishra_2021, Zajko_2022, Zhao_Wang_Yatskar_Ordonez_Chang_2017, binns2021, dacon2021does, rekabsaz2021, Chancellor_2019, Hutchinson2020socialbiases, phan2019amazon, Moore2020, Marda_Narayan_2020, tomalin2021practical, Tantipongpipat2019, samadi2018, BarocasSelbst_2016}  \\ \midrule
Stereotyping social groups & \cite{Abid_Farooqi_Zou_2021, Balayn_Lofi_Houben_2021, Bandy2021, binns2021, Birhane_Prabhu_Kahembwe_2021, Blodgett_Barocas_Daume_Wallach_2020, Cambre_Kulkarni_2019, Davis_Williams_Yang_2021, DeVos_Dhabalia_Shen_Holstein_Eslami_2022, Dev_Monajatipoor_Ovalle_Subramonian_Phillips_Chang_2021, Dobbe_Dean_Gilbert_Kohli_2018, Hendricks_Burns_Saenko_Darrell_Rohrbach_2018, Hutchinson_Prabhakaran_Denton_2020, Kaminski_Malgieri_2020, Katzman_Barocas_Blodgett_Laird_Scheuerman_Wallach_2021, Kay_Matuszek_Munson_2015, Liang_Li_Zheng_Lim_Salakhutdinov_Morency_2020, Lloyd_2018, Luccioni_Corry_Sridharan_Ananny_Schultz_Crawford_2022, Paullada_Raji_Bender_Denton_Hanna_2021, Savoldi_Gaido_Bentivogli_Negri_Turchi_2021, Sondergaard_Hansen_2018, Sweeney_2013, tomalin2021practical, vanEs_2021, Wang_Barocas_Laird_Wallach_2022, Weidinger2022, Yee_Tantipongpipat_Mishra_2021, Zhao_Wang_Yatskar_Ordonez_Chang_2017, microsoft_2020}  \\ \midrule
Demeaning social groups & \cite{Abid_Farooqi_Zou_2021, Blodgett_Barocas_Daume_Wallach_2020, Dobbe_Dean_Gilbert_Kohli_2018, Jane_2018, Katzman_Barocas_Blodgett_Laird_Scheuerman_Wallach_2021, Kay_Matuszek_Munson_2015, Keyes_2018, Lloyd_2018, Monroe-White_2021, Paullada_Raji_Bender_Denton_Hanna_2021, samadi2018, Sweeney_2013, Thiago_Marcelo_Gomes_2021, Wang_Barocas_Laird_Wallach_2022, Weidinger2022, Yee_Tantipongpipat_Mishra_2021}  \\ \midrule
Erasing social groups & \cite{Devinney_2022, Field_Blodgett_Waseem_Tsvetkov_2021, Katzman_Barocas_Blodgett_Laird_Scheuerman_Wallach_2021, Wang_Barocas_Laird_Wallach_2022, Weidinger2022}  \\ \midrule
Alienating social groups & \cite{Kay_Matuszek_Munson_2015, Wang_Barocas_Laird_Wallach_2022}  \\ \midrule
Denying opportunity to self-identify / non-consensual representations & \cite{Chancellor_2019, Devinney_2022, Katzman_Barocas_Blodgett_Laird_Scheuerman_Wallach_2021, Paullada_Raji_Bender_Denton_Hanna_2021, Wang_Barocas_Laird_Wallach_2022, Wang_Ramaswamy_Russakovsky_2022, Raji_Gebru_Mitchell_Buolamwini_Lee_Denton_2020}  \\ \midrule
Reifying essentialist social categories & \cite{Dobbe_Dean_Gilbert_Kohli_2018, Hanna_Denton_Smart_Smith-Loud_2020, Hoffmann_2021, Jane_2018, Katzman_Barocas_Blodgett_Laird_Scheuerman_Wallach_2021, Keyes_2018, Monroe-White_2021, phan2019amazon, Raji_Gebru_Mitchell_Buolamwini_Lee_Denton_2020, Sadowski_Selinger_2014, Sambasivan_Arnesen_Hutchinson_Doshi_Prabhakaran_2021, Spiel2019, Wang_Barocas_Laird_Wallach_2022, Welbl_2021} \\ \hline
\end{longtable}
\end{center}


==> tablesAndFigures/societaldatasources.tex <==
\newpage
\begin{center}
\begin{longtable}{{p{5cm}p{8cm}}}
\caption{Social system harms described in data sources.}
\label{societaldatasources}\\
\toprule
Sub-type & References  \\ \midrule

Social system harms (generally) & 
{Societal harms (generally):} \cite{Agrafiotis_Nurse_Goldsmith_Creese_Upton_2018, Agrafiotis_2016, Bengio_Beygelzimer_Crawford_Fromer_Gabriel_Levendowski_Raji_Ranzato_2022, microsoft_2020, Redden_Brand_2017, van_der_Sloot_van_Schendel_2021, CSETTaxonomy, Wardle_and_Derakhshan_2017}; Amplifying existing power disparities: \cite{Altman_Wood_Vayena_2018, Avila_2018, Bailey_Burkell_Dunn_Gosse_Steeves_2021, Bandy2021, Barabas_Doyle, barocas-hardt-narayanan, BarocasSelbst_2016, Bedford_Mann_Foth_Walters_2022, Benjamin_2019, Bennett_Gleason_Scheuerman_Bigham_Guo_To_2021, binns2021, Birhane_2021, Blodgett_Barocas_Daume_Wallach_2020, Buolamwini_Friedler_Wilson, Chi_Lurie_Mulligan, corry2021problem, Costanza-Chock_Raji_Buolamwini_2022, Davis_Williams_Yang_2021, Chancellor_2019, Dev_Monajatipoor_Ovalle_Subramonian_Phillips_Chang_2021, Dobbe_Krendl_Gilbert_Mintz_2021, Dosono_Semaan_2020, Dragiewicz_2018, Ehsan_Singh_Metcalf_Riedl_2022, Ekstrand_Das_Burke_Diaz_2022, Fazelpour_Lipton_2020, Field_Blodgett_Waseem_Tsvetkov_2021, Hendricks_Burns_Saenko_Darrell_Rohrbach_2018, Hoffmann_2021, Hutchinson_Prabhakaran_Denton_2020, Hutchinson2020socialbiases, Jacobs_2021, joyce2021toward, Karizat_2021, Karumbaiah_Brooks_2021, Katell_Young_Dailey_Herman_Guetler_Tam_Bintz_Raz_Krafft_2020, Knox_2019, Lloyd_2018, Malik_Viljanen_Lepinkainen_Alvesalo-Kuusi_Others, Mann_Matzner_2019, Markl_2022, McGlynn_Rackley_2017, Mohamed_Png_Isaac_2020, Moss_2021, Nedzhvetskaya_Tan_2021, Raji_Gebru_Mitchell_Buolamwini_Lee_Denton_2020, Ramesh_Kameswaran_Wang_Sambasivan_2022, Richardson_Gilbert_2021, Sambasivan_Arnesen_Hutchinson_Doshi_Prabhakaran_2021, Savoldi_Gaido_Bentivogli_Negri_Turchi_2021, Scheuerman_Jiang_Fiesler_Brubaker_2021, Shen_2021, Sloane_Moss_Awomolo_Forlano_2020, Smuha_2021b, Smuha_2021c, Suresh_Guttag_2021, Thiago_Marcelo_Gomes_2021, vanEs_2021, Weidinger2022, Weinberg_2022, Zajko_2022, Zhao_Wang_Yatskar_Ordonez_Chang_2017, Wang_2020, Metcalf_Moss_Watkins_Singh_Elish_2021} \\ \midrule

Information harms & Information harms (generally): \cite{Altman_Wood_Vayena_2018, CSETTaxonomy, Wardle_and_Derakhshan_2017}; Disinformation: \cite{Ekstrand_Das_Burke_Diaz_2022, janzen2022cognitive, Wardle_and_Derakhshan_2017, Wardle_Singerman_2021}; Distortion of reality: \cite{Altman_Wood_Vayena_2018, Bandy2021, Dosono_Semaan_2020, microsoft_2020}; Information asymmetries: \cite{Caplan_Gillespie_2020}; Malinformation: \cite{janzen2022cognitive, Wardle_and_Derakhshan_2017}; Misinformation: \cite{modei_Olah_Steinhardt_Christiano_Schulman_Mane_2016, Blodgett_Barocas_Daume_Wallach_2020, brundage2018malicious, Chancellor_2019, Ekstrand_Das_Burke_Diaz_2022, Katell_Young_Dailey_Herman_Guetler_Tam_Bintz_Raz_Krafft_2020, microsoft_2020, Neumann_De-Arteaga_Fazelpour_2022, Pendse2022, Smuha_2021c, Southwell_Brennen_Paquin_Boudewyns_Zeng_2022, Tran_Valecha_Rad_Rao_2020, Treen_Williams_ONeill_2020, Wardle_and_Derakhshan_2017, Wardle_Singerman_2021, Weidinger2022, Weinberg_2022, Wright_Williams_Elizarova_Dahne_Bian_Zhao_Tan_2021}; Subjugating and reshaping knowledge: \cite{DeVos_Dhabalia_Shen_Holstein_Eslami_2022, Sadowski_Selinger_2014, Singh_Joachims_2018}\\ \midrule

Cultural harms & Cultural harms (generally):
~\cite{DeVos_Dhabalia_Shen_Holstein_Eslami_2022, Dobbe_Dean_Gilbert_Kohli_2018, Irani_Vertesi_Dourish_Philip_Grinter_2010, Malik_Viljanen_Lepinkainen_Alvesalo-Kuusi_Others}; 
Cultural hegemony: ~\cite{Docherty_Biega_2022, Dosono_Semaan_2020}; Deteriorating social bonds: ~\cite{McGlynn_Rackley_2017}; Erasure: ~\cite{Devinney_2022, DeVos_Dhabalia_Shen_Holstein_Eslami_2022, Dosono_Semaan_2020, Keyes_2018, Sambasivan_Arnesen_Hutchinson_Doshi_Prabhakaran_2021}; Misinformation about social groups: ~\cite{Dosono_Semaan_2020, Sambasivan_Arnesen_Hutchinson_Doshi_Prabhakaran_2021} \\ \midrule

Political and civic harms & Political and civic harms (generally): ~\cite{Malik_Viljanen_Lepinkainen_Alvesalo-Kuusi_Others, Redden_Brand_2017, Satra_2020, Satra_2021, CSETTaxonomy}; Erosion of democracy (e.g., election interference, censorship, harm to civil liberties): ~\cite{Birhane_2021, corry2021problem, Green_Viljoen_2020, Lloyd_2018, microsoft_2020, Satra_2020, Satra_2021, Skirpan_Fiesler_2018, Smuha_2021b, Tufekci_Rit_Adam_Kramer_Guillory_Hancock, Moss_2021}; Human rights violations: \cite{Agrafiotis_2016, microsoft_2020, Moss_2021, Satra_2021, Sambasivan_Arnesen_Hutchinson_Doshi_Prabhakaran_2021, Yeung_Howes_Pogrebna}; Legal system harms (e.g., wrongful arrest, court transcription errors, unreasonable searches): ~\cite{modei_Olah_Steinhardt_Christiano_Schulman_Mane_2016, brundage2018malicious, Costanza-Chock_Raji_Buolamwini_2022, Dobbe_Dean_Gilbert_Kohli_2018, Feder_Cooper_Moss_Laufer_Nissenbaum_2022, koenecke2020racial, Mannes_2020, Redden_Brand_2017, Tufekci_Rit_Adam_Kramer_Guillory_Hancock, Moss_2021}; Nation destabilization (e.g., social polarization, loss of legitimacy): ~\cite{Agrafiotis_Nurse_Goldsmith_Creese_Upton_2018, Mohamed_Png_Isaac_2020, Satra_2020, Skirpan_Fiesler_2018, Smuha_2021b} \\ \midrule

Macro socio-economic harms & Macro socio-economic harms (generally): \cite{Agrafiotis_2016, Malik_Viljanen_Lepinkainen_Alvesalo-Kuusi_Others, Png_2022, Weidinger2022}; Algorithmic flash crashes: \cite{Agrafiotis_2016, Malik_Viljanen_Lepinkainen_Alvesalo-Kuusi_Others, Mohamed_Png_Isaac_2020}; Data harms: \cite{Mohamed_Png_Isaac_2020}; Digital divides: \cite{Ayodeji_Olamijuwon_Kokomma_Onyemelukwe_Gboyega_2021, Field_Blodgett_Waseem_Tsvetkov_2021, Irani_Vertesi_Dourish_Philip_Grinter_2010, microsoft_2020, Wang_Zhao_Van_Kleek_Shadbolt_2022, modei_Olah_Steinhardt_Christiano_Schulman_Mane_2016, galaz2021artificial};
Labor exploitation: \cite{Docherty_Biega_2022, microsoft_2020, Mohamed_Png_Isaac_2020};
Technological unemployment (e.g., professional displacement, disruption to livelihood, automation of tasks, devaluation of human expertise): \cite{Bengio_Beygelzimer_Crawford_Fromer_Gabriel_Levendowski_Raji_Ranzato_2022, cave2019bridging, joyce2021toward, microsoft_2020, Png_2022}; Worsening worker conditions: \cite{Bengio_Beygelzimer_Crawford_Fromer_Gabriel_Levendowski_Raji_Ranzato_2022}\\ \midrule

Environmental harms & Environmental harms: Ecological harms/depletion of natural resources: \cite{Bandy2021, Bedford_Mann_Foth_Walters_2022, microsoft_2020, Mohamed_Png_Isaac_2020, Png_2022, Smuha_2021c, Weidinger2022, Welbl_2021, Moss_2021, galaz2021machine}; 
Damage to built environment: \cite{Bandy2021, Mannes_2020, Smuha_2021b, CSETTaxonomy}; Injury to animals: \cite{Dean_Gilbert_Lambert_Zick_2021} \\ \hline
\end{longtable}
\end{center}

==> tablesAndFigures/sociotechnicalharmframework.tex <==
\begin{table}[ht]
\fontsize{7.2}{8.2}\selectfont
\centering
\setlength{\tabcolsep}{4.5pt}
\caption{Sociotechnical harm framework with specific harm types}
\resizebox*{\linewidth}{!}{
\begin{tabular}{p{2cm}p{4cm}p{10.5cm}}

\toprule
Harm Theme & Sub-Types & Specific Harms \\ \midrule
Representational & Stereotyping & Oversimplified and undesirable representations \\  \cline{2-3}
 & Demeaning social groups & Representations of a particular group as a lower social status using discourses, images, and language used to marginalize or oppress a social group \\  \cline{2-3}
 & Erasing social groups & Hegemonic ideas or social relations normalized in algorithmic systems \\ 
 &  & Systemic illegibility or absence of social groups in algorithmic system inputs/outputs \\ 
 &  & Unequal visibility of certain social groups \\  \cline{2-3}
 & Alienating social groups & Failure to acknowledge one’s membership in a culturally significant social group \\
 &  & Classifying or describing socially significant events in ways that ignores social injustices \\  \cline{2-3}
 & Denying opportunity to self-identify & Non-consensual classifications or representations of a person in algorithmic systems \\  \cline{2-3}
 & Reifying essentialist social \par categories & Reinforcing socially constructed categories as ‘natural’ \\  \hline
Allocative & Opportunity loss & Discrimination in critical resource domains (e.g., education, government, healthcare, or housing) \\
 &  & Inequitable access to resources needed to equitably participate in society \\  \cline{2-3}
 & Economic loss & Employment or hiring discrimination \\
 &  & Demonetization based on sensitive characteristics \\
 &  & Discrimination in  insurance, banking, or other financial sectors \\  
 &  & Financial losses or injuries, including price   discrimination \\  \hline
Quality-of-service & Alienation & Adverse emotions (e.g., frustration, bother, disappointment, or anger) experienced when interacting with technologies that fail based on one’s identity characteristics \\
 &  & Algorithmic invisibility, or feelings of exclusion from using non-inclusive technologies \\ \cline{2-3}
 & Increased labor & Additional effort required to make technologies operate as intended \\
 &  & Identity-based accommodation   to technologies (e.g., linguistic) \\
 &  & Wasted time/labor based on technology failures \\\cline{2-3}
 & Service or benefit loss & Degraded performance based on identity characteristics \\
 &  & Disproportionate loss of technological benefits \\ \hline
Interpersonal & Loss of agency or control & Algorithmically-informed identity change \\
 &  & Algorithmic profiling \\
 &  & Loss of autonomy \\
 &  & Required use of specific technologies to access domains that affect material well-being \\  \cline{2-3}
 & Tech-facilitated violence & Coercive control, or intimate partner violence \\
 &  & Device lockout and control \\
 &  & Inciting or enabling offline violence \\
 &  & Online abuse (e.g., cyberbullying, deadnaming, doxxing, trolling, hateful or toxic language, gender-based sexual harassment) \\  \cline{2-3}
 & Diminished health/well-being & Behavioral manipulation \\
 &  & Emotional harms (e.g., dignity loss, invalidation, misgendering, psychological harms) \\
 &  & Physical harms \\
 &  & Reputational harms \\  \cline{2-3}
 & Privacy violations & Exploitative or undesired inferences \\
 &  & Feelings of surveillance, or loss of desired anonymity \\
 &  & Loss of right to be forgotten \\
 &  & Non-consensual data collection \\
 &  & Privacy attacks (e.g., identity theft, doxxing) \\ \hline
Social/societal & Information harms & Disinformation \\
 &  & Distortion of reality (e.g., creation of information “bubbles”) \\
 &  & Malinformation \\
 &  & Misinformation \\
 &  & Subjugating knowledges or foreclosing alternative ways of knowing \\  \cline{2-3}
 & Cultural harms & Cultural hegemony \\
 &  & Deteriorating social bonds \\
 &  & Proliferating false perceptions about cultural groups \\
 &  & Systemic erasure of culturally significant objects and practices \\  \cline{2-3}
 & Political and civic harms & Erosion of democracy (e.g., election interference, censorship, harm to civil liberties) \\
 &  & Human rights violations \\
 &  & Legal system harms (e.g., wrongful arrest, court   transcription errors, unreasonable searches) \\
 &  & Nation destabilization (e.g., social   polarization, loss of legitimacy) \\  \cline{2-3}
 & Macro socio-economic harms & Digital divides \\
 &  & Labor exploitation \\
 &  & Systemic failures of financial systems \\
 &  & Technological unemployment (e.g., deskilling,   devaluation of human labor, or job displacement) \\  \cline{2-3}
 & Environmental harms & Damage to natural environment \\
 &  & Damage to built environment or property \\
 &  & Depletion or contamination of natural resources \\
 &  & Injury to animals \\ \hline
\end{tabular}}
\end{table}
